Selective Run-Length Encoding

Run-Length Encoding (RLE) is one of the most fundamental tools in data compression. However, its compression power drops significantly if there lacks consecutive elements in the sequence. In extreme cases, the output of the encoder may require more space than the input (aka size inflation). To alleviate this issue, using combinatorics, we quantify RLE's space savings for a given input distribution. With this insight, we develop the first algorithm that automatically identifies suitable symbols, then selectively encodes these symbols with RLE while directly storing the others without RLE. Through experiments on real-world datasets of various modalities, we empirically validate that our method, which maintains RLE's efficiency advantage, can effectively mitigate the size inflation dilemma.

==> tabs/old_results.tex <==
\setlength{\tabcolsep}{0.1cm}
\begin{table}[!t]\footnotesize
\centering
\subfloat[Mercari]{
\begin{tabular}{p{1.7cm}?>{\lcell}p{0.7cm}>{\rcell}p{1.05cm}|>{\lcell}p{0.7cm}>{\rcell}p{1.05cm}|>{\lcell}p{0.7cm}>{\rcell}p{1.05cm}?>{\lcell}p{0.7cm}>{\rcell}p{1.05cm}|>{\lcell}p{0.7cm}>{\rcell}p{1.05cm}|>{\lcell}p{0.7cm}>{\rcell}p{1.05cm}}
\toprule 
& \multicolumn{6}{c?}{Bit-packing} & \multicolumn{6}{c}{Variable-Length}\\ \cmidrule{2-13}
& \multicolumn{2}{c|}{\textsf{V-RLE}} & \multicolumn{2}{c|}{\textsf{D-RLE}} & \multicolumn{2}{c?}{\textsf{Ours}} & \multicolumn{2}{c|}{\textsf{V-RLE}} & \multicolumn{2}{c|}{\textsf{D-RLE}} & \multicolumn{2}{c}{\textsf{Ours}} \\ \midrule
\texttt{Condition} & \cellcolor{red!0}25.0 &\cellcolor{red!0}  [-8.9] &\cellcolor{red!0} 18.4 &\cellcolor{red!0} [-2.3] & \bftab 16.1 & [0.0] &  \cellcolor{red!0}33.3 & \cellcolor{red!0}[-4.9] & \cellcolor{red!0}28.6 &\cellcolor{red!0} [-0.2] & \bftab 28.4 & [0.0]\\ \midrule
\texttt{Category} & \cellcolor{red!0} 79.9 & \cellcolor{red!0}[-20.8] & \cellcolor{red!0}59.9 & \cellcolor{red!0}[-0.8] & \bftab 59.1 & [0.0] & \cellcolor{red!0}77.4 & \cellcolor{red!0}[-20.8] & \cellcolor{red!0}57.3 & \cellcolor{red!0}[-0.7] & \bftab 56.6 & [0.0] \\ \midrule
\texttt{Brand} & \cellcolor{red!0}74.2 & \cellcolor{red!0}[-4.3] & \cellcolor{green!0} \bftab 62.4 &\cellcolor{green!0} [7.5] & \cellcolor{green!0} \bftab 62.4 & \cellcolor{green!0}[7.5] & \cellcolor{red!0}56.3 & \cellcolor{red!0}[-12.3] & \cellcolor{red!0}44.3 & \cellcolor{red!0}[-0.3] & \bftab 44.0 & [0.0] \\ \midrule
\texttt{Shipping} & \cellcolor{red!0} 13.3 & \cellcolor{red!0}[-7.9] & \cellcolor{red!0}\textcolor{white}{0}9.1 & \cellcolor{red!0}[-3.7] & \bftab \textcolor{white}{0}5.4 & [0.0] & \cellcolor{green!0} \bftab 23.9 & \cellcolor{green!0}[3.0] & \cellcolor{green!0}24.0 & \cellcolor{green!0}[2.9] & \cellcolor{green!0} \bftab 23.9 & \cellcolor{green!0}[3.0] \\
                           \bottomrule
\end{tabular}
\label{stab:mercari}
}

\subfloat[Netstream]{
\begin{tabular}{p{1.7cm}?>{\lcell}p{0.7cm}>{\rcell}p{1.05cm}|>{\lcell}p{0.7cm}>{\rcell}p{1.05cm}|>{\lcell}p{0.7cm}>{\rcell}p{1.05cm}?>{\lcell}p{0.7cm}>{\rcell}p{1.05cm}|>{\lcell}p{0.7cm}>{\rcell}p{1.05cm}|>{\lcell}p{0.7cm}>{\rcell}p{1.05cm}}
\toprule 
& \multicolumn{6}{c?}{Bit-packing} & \multicolumn{6}{c}{Variable-Length}\\ \cmidrule{2-13}
& \multicolumn{2}{c|}{\textsf{V-RLE}} & \multicolumn{2}{c|}{\textsf{D-RLE}} & \multicolumn{2}{c?}{\textsf{Ours}} & \multicolumn{2}{c|}{\textsf{V-RLE}} & \multicolumn{2}{c|}{\textsf{D-RLE}} & \multicolumn{2}{c}{\textsf{Ours}} \\ \midrule
\texttt{Src\_IP} & 409.5 &[-68.3] & 364.6 & [-23.4] & 341.2 &[0.0] & 426.5 & [-41.7] & 429.8 &[-45.0] & 384.8 &[0.0]\\ \midrule
\texttt{Dst\_IP} & 384.9 &[-60.1] & 308.4 &[16.4] & 303.5 & [21.3] & 428.5 &[-76.5] & 421.6 & [-69.6] & 352.0 & [0.0]\\ \midrule
\texttt{Src\_Port} & 282.3 &[-9.3] & 292.6 &[-19.6] & 273.0 & [0.0] & 315.4 & [-25.9] & 304.2 &[-14.7] & 289.5 &[0.0]\\ \midrule
\texttt{Dst\_Port} & 227.0 &[-36.0] & 205.8 &[-14.8] & 191.0 &[0.0] & 206.2 &[24.6] & 213.6 &[17.2] &  198.0 &[32.8]\\ \midrule
\texttt{Protocol} & \textcolor{white}{0}63.2 &[13.1] & \textcolor{white}{0}65.5 &[10.8] & \textcolor{white}{0}63.2 &[13.1] & \textcolor{white}{0}68.0 &[3.3] & \textcolor{white}{0}60.7 &[7.3] & \textcolor{white}{0}60.7 &[7.3]\\
                           \bottomrule
\end{tabular}\label{stab:netstream}
}
\caption{Column size (MB) of SO-2018 after encoding. For each representation method, the smallest size is highlighted in {\bftab bold}. We additionally calculate the reduced size (see the square bracket on the right of a cell).}
% with positive and negative reductions respectively coloured in \colorbox{green!0}{green} and \colorbox{red!0}{red}.}
\end{table}
